TARDiS : Text Augmentation for Refining Diversity and Separability

Text augmentation (TA) is a critical technique for text classification, especially in few-shot settings. This paper introduces a novel LLM-based TA method, TARDiS, to address challenges inherent in the generation and alignment stages of two-stage TA methods. For the generation stage, we propose two generation processes, SEG and CEG, incorporating multiple class-specific prompts to enhance diversity and separability. For the alignment stage, we introduce a class adaptation (CA) method to ensure that generated examples align with their target classes through verification and modification. Experimental results demonstrate TARDiS's effectiveness, outperforming state-of-the-art LLM-based TA methods in various few-shot text classification tasks. An in-depth analysis confirms the detailed behaviors at each stage.

==> table/table2.tex <==
\begin{tabular}{lcccccc}
\toprule
                        & \multicolumn{2}{c}{\textbf{BANKING77}}            & \multicolumn{2}{c}{\textbf{CLINC150}}             & \multicolumn{2}{c}{\textbf{HWU64}}                \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
\multicolumn{1}{c}{}    & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{10}    & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{10}    & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{10}    \\ \midrule
\multicolumn{7}{c}{\texttt{Roberta-base}}                                                                                                                                           \\ \midrule
baseline                & 74.38                 & 82.11                     & 87.99                 & 91.55                     & 75.56                 & 82.90                     \\
Static Prompt &                  &                      &                  &                      &                  &                     \\
Static Prompt + CA                &                  &                      &                  &                      &                  &                     \\
DNNC                    & 80.40                 & 86.71                     & 91.02                 & 93.76                     & 80.46                 & 84.72                     \\
CPFT                    & 80.86                 & 87.20                     & 92.34                 & 94.18                     & 82.03                 & \textbf{87.13}            \\
TARDiS                  & \textbf{83.50}        & \textbf{87.30}            & \textbf{93.34}        & \textbf{94.96}            & \textbf{83.42}        & 86.52                     \\ \midrule
\multicolumn{7}{c}{\texttt{Roberta-large}}                                                                                                                                          \\ \midrule
baseline                & 80.32                 & 86.52                     & 89.89                 & 93.56                     & 79.18                 & 84.11                     \\
Static Prompt &           82.50    &                      &                  &                      &                  &                     \\
Static Prompt + CA                &            84.04            &                      &                  &                      &                  &                     \\
ICDA                    & 84.01                 & \textbf{89.79}            & 92.62                 & 94.84                     & 82.45                 & 87.41                     \\
TARDiS                  & \textbf{85.34}        & 88.89                     & \textbf{94.24}        & \textbf{95.02}            & \textbf{84.45}        &\textbf{87.52}             \\ 
\bottomrule
\end{tabular}

==> table/table4.tex <==
\begin{tabular}{l|ccc|l}
\toprule
    & \textbf{SEG}  & \textbf{CEG}  & \textbf{CA}                   & \multicolumn{1}{c}{\textbf{Accuracy}}     \\ 
    \midrule
(a)   & \checkmark    & \checkmark    & \checkmark                    & \textbf{85.45}                            \\
(b)   & \checkmark    & \checkmark    &                               & 79.98 (-5.47)                             \\
(c)   & \checkmark    &               & \checkmark                    & 84.67 (-0.78)                             \\
(d)   &     &  \checkmark             & \checkmark                    & 84.64 (-0.81)                             \\
(e)   &    &  $\triangle$             & \checkmark                    & 82.23 (-3.22)                             \\
\midrule
(f)   & & & & 80.32 (-5.13) \\
\bottomrule
\end{tabular}

==> table/table7.tex <==
\begin{tabular}{l|l}
\toprule
(a) & What's the quickest way \hl{to get}  to LaGuardia from here? 
\\ & $\Rightarrow$ What's the fastest way \hl{to hail a taxi} to LaGuardia from here? \\
\midrule
(b) & Where can I \hl{~~~} \\
& $\Rightarrow$ Where can I \hl{find a reliable taxi service} \\
\midrule
(c) & How \hl{long} will it take to reach Brooklyn Bridge from Times Square \hl{by taxi?} \\
& $\Rightarrow$ How \hl{much} time will it take to get to Brooklyn Bridge from Times Square \hl{by hailing a taxi?} \\
\bottomrule
\end{tabular}
